The renormalised $\mathrm{O}(a)$ improved vector current in three-flavour lattice QCD with Wilson quarks

We present the results of a non-perturbative determination of the improvement coefficient $c_\mathrm{V}$ and the renormalisation factor $Z_\mathrm{V}$, which define the renormalised vector current in three-flavour $\mathrm{O}(a)$ improved lattice QCD with Wilson quarks and tree-level Symanzik-improved gauge action. In case of the improvement coefficient, we consider both lattice descriptions of the vector current, the local as well as the conserved (i.e., point-split) one. Our improvement and normalisation conditions are based on massive chiral Ward identities and numerically evaluated in the Schr\"odinger functional setup, which allows to eliminate finite quark mass effects in a controlled way. In order to ensure a smooth dependence of the renormalisation constant and improvement coefficients on the bare gauge coupling, our computation proceeds along a line of constant physics, covering the typical range of lattice spacings $0.04\,\mathrm{fm}\lesssim a\lesssim 0.1\,\mathrm{fm}$ that is useful for phenomenological applications. Especially for the improvement coefficient of the local vector current, we report significant differences between the one-loop perturbative estimates and our non-perturbative results.

==> 02_ensembles.tex <==
\section{Numerical investigation}
The parameters for the gauge field ensembles used in this study  are summarized in table \ref{tab:gauge_parameters}. The ensembles are designed to lay on a line of constant physics defined by a physical extent $L\approx1.1\,$fm. As the original tuning was based on the perturbative 2-loop beta function as explained in \cite{Bulava:2015bxa}, $L$ is only constant up to cutoff effects. We explicitly checked the cutoff effects with the results of \cite{Bruno:2016plf} and found that their are consistent with $\mathrm{O}(a)$. We thus expect that our results are only affected at $\mathrm{O}(a^2)$ for the renormalization constant and $\mathrm{O}(a)$ for the improvement coefficients, which is beyond our required precision and is treated as an additional ambiguity which has not be accounted for in the final error budget.
The gauge ensembles which are he basis for the numerical results in this study where already used in \cite{Bulava:2015bxa,Bulava:2016ktf,Heitger:2017njs,Heitger:2018pwb,deDivitiis:2019xla,Chimirri:2019xsv}. 

\begin{table}[t]
	\centering
	\renewcommand{\arraystretch}{1.25}
	\setlength{\tabcolsep}{3pt}
	\begin{tabular}{ccllrrcl}
		\toprule
		ID     & $L^3\times T/a^4$   &   $\beta$ &   $\kappa$ &   $N$ &   $N_r$ &   $P(Q_0)$ & $\tau_\mathrm{exp}$   \\
		\midrule
		 A1k1     & $12^3\times 17$     &     3.3   &   0.13652  &  2560 &      20 &      0.365 & 1.031(71)             \\
		A1k3     & $12^3\times 17$     &     3.3   &   0.13648  &  1719 &       5 &      0.357 & 2.06(14)              \\
		A1k4     & $12^3\times 17$     &     3.3   &   0.1365   & 12080 &      20 &      0.366 & 1.031(71)             \\
		\midrule
		E1k1     & $14^3\times 21$     &     3.414 &   0.1369   &  4800 &      32 &      0.353 & 1.61(12)              \\
		E1k2     & $14^3\times 21$     &     3.414 &   0.13695  &  7200 &      48 &      0.375 & 1.61(12)              \\
		\midrule
		B1k1     & $16^3\times 23$     &     3.512 &   0.137    &  2560 &       2 &      0.389 & 4.41(96)              \\
		B1k2     & $16^3\times 23$     &     3.512 &   0.13703  &  1024 &       1 &      0.341 & 4.41(96)              \\
		B1k3     & $16^3\times 23$     &     3.512 &   0.1371   &  2048 &       2 &      0.458 & 4.41(96)              \\
		B1k4     & $16^3\times 23$     &     3.512 &   0.13714  &  3482 &       1 &      0.402 & 4.41(96)              \\
		\midrule
		C1k1     & $20^3\times 29$     &     3.676 &   0.1368   &   981 &       1 &      0.334 & 10.7(4.1)             \\
		C1k2     & $20^3\times 29$     &     3.676 &   0.137    &  1904 &       4 &      0.450  & 10.7(4.1)             \\
		C1k3     & $20^3\times 29$     &     3.676 &   0.13719  &  1934 &       4 &      0.645 & 10.7(4.1)             \\
		\midrule
		D1k2     & $24^3\times 35$     &     3.81  &   0.13701  &   803 &       2 &      0.445 & 62(14)                \\
		D1k4     & $24^3\times 35$     &     3.81  &   0.137033 &  5313 &       8 &      0.653 & 31(7)             \\
		\bottomrule
	\end{tabular}
	\caption{Summary of simulation parameters for the gauge configuration ensembles labeled by `ID'. $N$ denotes the number of configurations for each ensemble, $N_\mathrm{r}$ the number of replica. $P(Q_0)$ labels the percentage of configurations for which the topological charge $Q$ vanishes. $\tau_\mathrm{exp}$ describes the exponential autocorrelation time used for the tail in the data analysis. It is estimated from the integrated autocorrelation time of $Q^2$ on the longest Monte Carlo chain for each value of $\beta$. All ensembles are separated by $8$ molecular dynamics units, except for ensembles A1k3 (4) and D1k4 (16). This is the reason for the differing value of $\tau_\mathrm{exp}$ for these ensembles.}
	\label{tab:gauge_parameters}
\end{table}

For the finer lattice spacings our simulations are subject to critical slowing down of the topological charge $Q$. To make sure that an incorrect sampling of the topological charge does not affect our results, we project expectation values to the topologically trivial sector by reweighting as suggested in \cite{Fritzsch:2013yxa}.

For the error analysis we use a python implementation of the $\Gamma$-method with critical slowing down \cite{Wolff:2003sm,Schaefer:2010hu} with features similar to the ones described in \cite{Ramos:2018vgu}.
As estimate for the autocorrelation time $\tau_\mathrm{exp}$ of the slowest mode in a given Monte Carlo history we us the integrated autocorrelation time of $Q^2$, based on the assumption that due to the parity invariance of the HMC algorithm, it is sufficient to look for the slowest mode in parity even Observables \cite{Schaefer:2010hu}. We determine $\tau_\mathrm{exp}$ for the longest Monte Carlo chain available for each value of $\beta$ and use that result for the remaining ensembles, possibly adjusted by a factor stemming from different configuration spacings in MDU as shown in table \ref{tab:gauge_parameters}.
